Uncovering symmetric and asymmetric species associations from community and environmental data

There is no much doubt that biotic interactions shape community assembly and ultimately the spatial co-variations between species. There is a hope that the signal of these biotic interactions can be observed and retrieved by investigating the spatial associations between species while accounting for the direct effects of the environment. By definition, biotic interactions can be both symmetric and asymmetric. Yet, most models that attempt to retrieve species associations from co-occurrence or co-abundance data internally assume symmetric relationships between species. Here, we propose and validate a machine-learning framework able to retrieve bidirectional associations by analyzing species community and environmental data. Our framework (1) models pairwise species associations as directed influences from a source to a target species, parameterized with two species-specific latent embeddings: the effect of the source species on the community, and the response of the target species to the community; and (2) jointly fits these associations within a multi-species conditional generative model with different modes of interactions between environmental drivers and biotic associations. Using both simulated and empirical data, we demonstrate the ability of our framework to recover known asymmetric and symmetric associations and highlight the properties of the learned association networks. By comparing our approach to other existing models such as joint species distribution models and probabilistic graphical models, we show its superior capacity at retrieving symmetric and asymmetric interactions. The framework is intuitive, modular and broadly applicable across various taxonomic groups.

==> box_AlpsHSMw.tex <==
\renewcommand{\datafile}{xps/data_AlpsHSMw.csv}
\begin{tikzpicture}%[trim axis left, trim axis right]
\begin{axis}[width = .6\textwidth, height = 0.3\textwidth,
  ytick={1,2,3,4,5,6,7,8},
  yticklabels={\trtForm,\trtAspect,\trtZoogD,\trtPhysD,\trtSnow,\trtSlope},
  % yticklabels={\trtSlope,\trtSnow,\trtPhysD,\trtZoogD,\trtAspect,\trtForm},
  % x tick label style = {rotate=40, anchor=north, xshift=-2pt},
  % x tick label style = {font=\footnotesize},
  x label style = {yshift=5pt},
  y label style = {yshift=-2pt},
  % ytick={0,0.1,0.2},  
  % yticklabels={$0$,$0.1$,$0.2$},
  xmin=-9,
  xmax=9,
  % xmin=0.5,
  % xmax=8.5,
  boxplot/draw direction=x,
  cycle list name=divBlue,
  xlabel = {weight}, ylabel = {}
]
% \foreach \x/\c in {{Slope}/{3},{Snow}/{4},{PhysD}/{2},{ZoogD}/{5},{Aspect}/{0},{Form}/{1}}{
\foreach \x/\c in {{Form}/{1},{Aspect}/{0},{ZoogD}/{5},{PhysD}/{2},{Snow}/{4},{Slope}/{3}}{
  \addplot +[boxplot] table [y index=\c, col sep=comma] {\datafile};
}
\end{axis}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "tikz_figures"
%%% End:


==> grid_simul.tex <==
%\begin{table}[]
%	\begin{tabular}{|l|l|l|l|l|l|l|}
%		\hline
%		\textbf{Simulation ID} & \textbf{Selected dimension} & \textbf{Deviance of predicted abundance} & \textbf{Association types} & \textbf{Density} & \textbf{Poolsize} & \textbf{Directionality} \\ \hline
%		1                      & \textbf{2}                  & \textbf{0.88$\pm$0.88}                      & A                          & NA               & 5                 & NA                      \\ \hline
%		2                      & 2                           & 0.81$\pm$0.56                               & A                          & NA               & 10                & NA                      \\ \hline
%		2                      & \textbf{3}                  & \textbf{0.78$\pm$0.54}                      & A                          & NA               & 10                & NA                      \\ \hline
%		2                      & 5                           & 0.83$\pm$0.71                               & A                          & NA               & 10                & NA                      \\ \hline
%		3                      & 3                           & 0.84$\pm$0.39                               & A                          & NA               & 20                & NA                      \\ \hline
%		3                      & \textbf{5}                  & \textbf{0.83$\pm$0.4}                       & A                          & NA               & 20                & NA                      \\ \hline
%		3                      & 7                           & 0.83$\pm$0.41                               & A                          & NA               & 20                & NA                      \\ \hline
%		3                      & 9                           & 0.83$\pm$0.41                               & A                          & NA               & 20                & NA                      \\ \hline
%		4                      & \textbf{2}                  & \textbf{0.7$\pm$0.74}                       & A+F                        & Sparse           & 5                 & Symetric                \\ \hline
%		5                      & \textbf{2}                  & \textbf{0.46$\pm$0.59}                      & A+F                        & Dense            & 5                 & Symetric                \\ \hline
%		6                      & 2                           & 0.82$\pm$0.65                               & A+F                        & Sparse           & 10                & Symetric                \\ \hline
%		6                      & 3                           & 0.8$\pm$0.65                                & A+F                        & Sparse           & 10                & Symetric                \\ \hline
%		6                      & \textbf{5}                  & \textbf{0.71$\pm$0.6}                       & A+F                        & Sparse           & 10                & Symetric                \\ \hline
%		7                      & 2                           & 0.68$\pm$0.46                               & A+F                        & Dense            & 10                & Asymetric               \\ \hline
%		7                      & \textbf{4}                  & \textbf{0.63$\pm$0.47}                      & A+F                        & Dense            & 10                & Asymetric               \\ \hline
%		8                      & 2                           & 0.74$\pm$0.47                               & A+F                        & Sparse           & 10                & Symetric                \\ \hline
%		8                      & 3                           & 0.67$\pm$0.4                                & A+F                        & Sparse           & 10                & Symetric                \\ \hline
%		8                      & \textbf{5}                  & \textbf{0.66$\pm$0.4}                       & A+F                        & Sparse           & 10                & Symetric                \\ \hline
%		9                      & 2                           & 0.54$\pm$0.63                               & A+F                        & Dense            & 10                & Asymetric               \\ \hline
%		9                      & \textbf{4}                  & \textbf{0.44$\pm$0.43}                      & A+F                        & Dense            & 10                & Asymetric               \\ \hline
%		10                     & 3                           & 0.84$\pm$0.42                               & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		10                     & 5                           & 0.8$\pm$0.33                                & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		10                     & \textbf{7}                  & \textbf{0.79$\pm$0.32}                      & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		10                     & 9                           & 0.8$\pm$0.33                                & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		11                     & 2                           & 0.97$\pm$0.76                               & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		11                     & 3                           & 0.8$\pm$0.65                                & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		11                     & 4                           & 0.88$\pm$0.8                                & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		11                     & \textbf{8}                  & \textbf{0.75$\pm$0.54}                      & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		11                     & 9                           & 0.75$\pm$0.52                               & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		12                     & 3                           & 0.86$\pm$0.4                                & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		12                     & 5                           & 0.85$\pm$0.44                               & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		12                     & 7                           & 0.82$\pm$0.4                                & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		12                     & \textbf{9}                  & \textbf{0.79$\pm$0.35}                      & A+F                        & Sparse           & 20                & Symetric                \\ \hline
%		13                     & 2                           & 1.17$\pm$0.85                               & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		13                     & 3                           & 1.09$\pm$1.03                               & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		13                     & 4                           & 1.02$\pm$0.76                               & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		13                     & \textbf{8}                  & \textbf{0.82$\pm$0.76}                      & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		13                     & 9                           & 0.96$\pm$1.19                               & A+F                        & Dense            & 20                & Asymetric               \\ \hline
%		14                     & \textbf{2}                  & \textbf{1.25$\pm$0.88}                      & A+C                        & Sparse           & 5                 & Symetric                \\ \hline
%		15                     & \textbf{2}                  & \textbf{1.25$\pm$1.13}                      & A+C                        & Dense            & 5                 & Symetric                \\ \hline
%		16                     & 2                           & 1.16$\pm$0.65                               & A+C                        & Sparse           & 10                & Symetric                \\ \hline
%		16                     & 3                           & 1.07$\pm$0.66                               & A+C                        & Sparse           & 10                & Symetric                \\ \hline
%		16                     & \textbf{5}                  & \textbf{1.04$\pm$0.67}                      & A+C                        & Sparse           & 10                & Symetric                \\ \hline
%		17                     & 2                           & 0.92$\pm$0.65                               & A+C                        & Dense            & 10                & Asymetric               \\ \hline
%		17                     & \textbf{4}                  & \textbf{0.88$\pm$0.61}                      & A+C                        & Dense            & 10                & Asymetric               \\ \hline
%		18                     & 2                           & 1.17$\pm$0.67                               & A+C                        & Sparse           & 10                & Symetric                \\ \hline
%		18                     & 3                           & 1.1$\pm$0.73                                & A+C                        & Sparse           & 10                & Symetric                \\ \hline
%		18                     & \textbf{5}                  & \textbf{0.96$\pm$0.57}                      & A+C                        & Sparse           & 10                & Symetric                \\ \hline
%		19                     & 2                           & 1.15$\pm$0.8                                & A+C                        & Dense            & 10                & Asymetric               \\ \hline
%		19                     & \textbf{4}                  & \textbf{1.02$\pm$0.79}                      & A+C                        & Dense            & 10                & Asymetric               \\ \hline
%		20                     & 3                           & 0.78$\pm$0.31                               & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		20                     & \textbf{5}                  & \textbf{0.78$\pm$0.3}                       & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		20                     & 7                           & 0.78$\pm$0.32                               & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		20                     & 9                           & 0.78$\pm$0.32                               & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		21                     & 2                           & 0.94$\pm$0.52                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		21                     & 3                           & 0.87$\pm$0.51                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		21                     & 4                           & 0.86$\pm$0.49                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		21                     & 8                           & 0.85$\pm$0.48                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		21                     & \textbf{9}                  & \textbf{0.83$\pm$0.45}                      & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		22                     & 3                           & 0.97$\pm$0.61                               & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		22                     & 5                           & 0.96$\pm$0.58                               & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		22                     & \textbf{7}                  & \textbf{0.94$\pm$0.55}                      & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		22                     & 9                           & 0.95$\pm$0.51                               & A+C                        & Sparse           & 20                & Symetric                \\ \hline
%		23                     & 2                           & 0.98$\pm$0.51                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		23                     & 3                           & 0.89$\pm$0.47                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		23                     & 4                           & 0.89$\pm$0.48                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		23                     & \textbf{8}                  & \textbf{0.87$\pm$0.48}                      & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		23                     & 9                           & 0.87$\pm$0.48                               & A+C                        & Dense            & 20                & Asymetric               \\ \hline
%		24                     & \textbf{2}                  & \textbf{0.69$\pm$0.85}                      & A+F+C                      & Sparse           & 5                 & Symetric                \\ \hline
%		25                     & \textbf{2}                  & \textbf{0.79$\pm$0.86}                      & A+F+C                      & Dense            & 5                 & Symetric                \\ \hline
%		26                     & 2                           & 0.82$\pm$0.6                                & A+F+C                      & Sparse           & 10                & Symetric                \\ \hline
%		26                     & 3                           & 0.7$\pm$0.58                                & A+F+C                      & Sparse           & 10                & Symetric                \\ \hline
%		26                     & \textbf{5}                  & \textbf{0.67$\pm$0.51}                      & A+F+C                      & Sparse           & 10                & Symetric                \\ \hline
%		27                     & 2                           & 1.07$\pm$0.78                               & A+F+C                      & Dense            & 10                & Symetric                \\ \hline
%		27                     & 3                           & 0.98$\pm$0.71                               & A+F+C                      & Dense            & 10                & Symetric                \\ \hline
%		27                     & \textbf{5}                  & \textbf{0.9$\pm$0.7}                        & A+F+C                      & Dense            & 10                & Symetric                \\ \hline
%		28                     & 3                           & 0.8$\pm$0.31                                & A+F+C                      & Sparse           & 20                & Symetric                \\ \hline
%		28                     & 5                           & 0.8$\pm$0.33                                & A+F+C                      & Sparse           & 20                & Symetric                \\ \hline
%		28                     & \textbf{7}                  & \textbf{0.78$\pm$0.32}                      & A+F+C                      & Sparse           & 20                & Symetric                \\ \hline
%		28                     & 9                           & 0.79$\pm$0.33                               & A+F+C                      & Sparse           & 20                & Symetric                \\ \hline
%		29                     & 3                           & 0.86$\pm$0.44                               & A+F+C                      & Dense            & 20                & Symetric                \\ \hline
%		29                     & 5                           & 0.85$\pm$0.42                               & A+F+C                      & Dense            & 20                & Symetric                \\ \hline
%		29                     & 7                           & 0.85$\pm$0.44                               & A+F+C                      & Dense            & 20                & Symetric                \\ \hline
%		29                     & \textbf{9}                  & \textbf{0.83$\pm$0.4}                       & A+F+C                      & Dense            & 20                & Symetric                \\ \hline
%	\end{tabular}
%\caption{Embedding dimension selection based on minimal deviances of predicted abundances for each simulation. }
%\label{dimselsim}
%\end{table}


\begin{table}[H]
	\begin{tabularx}{\textwidth}{|s|b|s|b|b|b|b|}
		\hline
		\textbf{Sim. ID} & \textbf{Association types} & \textbf{Pool size} & \textbf{Density} & \textbf{Direction} & \textbf{Dimension} & \textbf{Deviance of predictions} \\ \hline
		1                      & A                          & 5                 & /                & /                       & \textbf{2}                  & \textbf{0.88$\pm$0.88}                       \\ \hline
		2                      & A                          & 10                & /                & /                       & \textbf{3}                  & \textbf{0.78$\pm$0.54}                       \\ \hline
		3                      & A                          & 20                & /                & /                       & \textbf{5}                  & \textbf{0.83$\pm$0.4}                        \\ \hline
		4                      & A+F                        & 5                 & Sparse           & Symetric                & \textbf{2}                  & \textbf{0.7$\pm$0.74}                        \\ \hline
		5                      & A+F                        & 5                 & Dense            & Symetric                & \textbf{2}                  & \textbf{0.46$\pm$0.59}                       \\ \hline
		6                      & A+F                        & 10                & Sparse           & Symetric                & \textbf{5}                  & \textbf{0.71$\pm$0.6}                        \\ \hline
		7                      & A+F                        & 10                & Sparse           & Asymetric               & \textbf{4}                  & \textbf{0.63$\pm$0.47}                       \\ \hline
		8                      & A+F                        & 10                & Dense            & Symetric                & \textbf{5}                  & \textbf{0.66$\pm$0.4}                        \\ \hline
		9                      & A+F                        & 10                & Dense            & Asymetric               & \textbf{4}                  & \textbf{0.44$\pm$0.43}                       \\ \hline
		10                     & A+F                        & 20                & Sparse           & Symetric                & \textbf{7}                  & \textbf{0.79$\pm$0.32}                       \\ \hline
		11                     & A+F                        & 20                & Sparse           & Asymetric               & \textbf{8}                  & \textbf{0.75$\pm$0.54}                       \\ \hline
		12                     & A+F                        & 20                & Dense            & Symetric                & \textbf{9}                  & \textbf{0.79$\pm$0.35}                       \\ \hline
		13                     & A+F                        & 20                & Dense            & Asymetric               & \textbf{8}                  & \textbf{0.82$\pm$0.76}                       \\ \hline
		14                     & A+C                        & 5                 & Sparse           & Symetric                & \textbf{2}                  & \textbf{1.25$\pm$0.88}                       \\ \hline
		15                     & A+C                        & 5                 & Dense            & Symetric                & \textbf{2}                  & \textbf{1.25$\pm$1.13}                       \\ \hline
		16                     & A+C                        & 10                & Sparse           & Symetric                & \textbf{5}                  & \textbf{1.04$\pm$0.67}                       \\ \hline
		17                     & A+C                        & 10                & Sparse           & Asymetric               & \textbf{4}                  & \textbf{0.88$\pm$0.61}                       \\ \hline
		18                     & A+C                        & 10                & Dense            & Symetric                & \textbf{5}                  & \textbf{0.96$\pm$0.57}                       \\ \hline
		19                     & A+C                        & 10                & Dense            & Asymetric               & \textbf{4}                  & \textbf{1.02$\pm$0.79}                       \\ \hline
		20                     & A+C                        & 20                & Sparse           & Symetric                & \textbf{5}                  & \textbf{0.78$\pm$0.3}                        \\ \hline
		21                     & A+C                        & 20                & Sparse           & Asymetric               & \textbf{9}                  & \textbf{0.83$\pm$0.45}                       \\ \hline
		22                     & A+C                        & 20                & Dense            & Symetric                & \textbf{7}                  & \textbf{0.94$\pm$0.55}                       \\ \hline
		23                     & A+C                        & 20                & Dense            & Asymetric               & \textbf{8}                  & \textbf{0.87$\pm$0.48}                       \\ \hline
		24                     & A+F+C                      & 5                 & Sparse           & Symetric                & \textbf{2}                  & \textbf{0.69$\pm$0.85}                       \\ \hline
		25                     & A+F+C                      & 5                 & Dense            & Symetric                & \textbf{2}                  & \textbf{0.79$\pm$0.86}                       \\ \hline
		26                     & A+F+C                      & 10                & Sparse           & Symetric                & \textbf{5}                  & \textbf{0.67$\pm$0.51}                       \\ \hline
		27                     & A+F+C                      & 10                & Dense            & Symetric                & \textbf{5}                  & \textbf{0.9$\pm$0.7}                         \\ \hline
		28                     & A+F+C                      & 20                & Sparse           & Symetric                & \textbf{7}                  & \textbf{0.78$\pm$0.32}                       \\ \hline
		29                     & A+F+C                      & 20                & Dense            & Symetric                & \textbf{9}                  & \textbf{0.83$\pm$0.4}                        \\ \hline
	\end{tabularx}
	\caption{Selected embedding dimension and its corresponding deviance over predicted abundances for each simulation. }
	\label{dimselsim}
\end{table}

==> network_summary.tex <==
\newcommand\myoff{2.}
\newcommand\mxoff{2.4}

\begin{tikzpicture}
  %\node at ({-1.5*\mxoff}, {-1.5*\myoff}) {North slope};
  \node[lightgray] at ({-1.*\mxoff}, {-3.1*\myoff}) {\textsc{\textbf{north slope}}};
  \node[lightgray] at ({1.*\mxoff}, {-3.1*\myoff}) {\textsc{\textbf{south slope}}};
  \draw[line width=5pt, lightgrey, opacity=0.5] ({-1.5*\mxoff}, {-1.5*\myoff}) -- ({0*\mxoff}, {0*\myoff}) -- ({3.2*\mxoff}, {-3.2*\myoff});
  % \node[rll node, TolRbwA] (msgras) at ({-0.02*\mxoff}, {0*\myoff}) {MS grassland};
  % \node[rll node, TolRbwA] (hsforb) at ({1.02*\mxoff}, {0*\myoff}) {HS forbs};
  % \node[rll node, TolRbwA] (domgra) at ({2*\mxoff}, {.5*\myoff}) {Dominant graminoids};
  % \node[rll node, TolRbwD] (dwashr) at ({2*\mxoff}, {-.5*\myoff}) {Dwarf shrubs};
  % \node[rll node, TolRbwF] (lsgras) at ({-1*\mxoff}, {-.5*\myoff}) {LS grassland};
  % \node[rll node, TolRbwF] (shoher) at ({-2.04*\mxoff}, {-.5*\myoff}) {Short herbs};
  % \node[rll node, TolRbwJ] (chinop) at ({-1*\mxoff}, {.5*\myoff}) {Chinopholous vegetation};
  % \path[pil]
  % (domgra) edge[drP, out=245,in=5,looseness=1] (hsforb)
  % (dwashr) edge[drP, out=115,in=355,looseness=1] (hsforb)
  % % (msgras) edge[drN, out=295, in=245,looseness=.6] (hsforb)
  % (msgras) edge[drN, out=65, in=115,looseness=.6] (hsforb)  
  % (msgras) edge[drN, in=65,out=185,looseness=1] (lsgras)
  % (msgras) edge[drN, in=295,out=175,looseness=1] (chinop)
  % (lsgras) edge[drN, in=65,out=115,looseness=.6] (shoher)
  % (msgras) edge[drN,loop above,looseness=4] (msgras)
  % (shoher) edge[drP,loop above,looseness=4] (shoher)
  % (chinop) edge[drP,loop below,looseness=4] (chinop);
  \node[TolRbwA, rll node] (msgras) at ({1.5*\mxoff}, {-1.5*\myoff}) {MS grassland};
  \node[TolRbwA, rll node] (hsforb) at ({.5*\mxoff}, {-.5*\myoff}) {HS forbs};
  \node[TolRbwA, rll node] (domgra) at ({0*\mxoff}, {0*\myoff}) {Dominant graminoids};
  \node[TolRbwD, rll node] (dwashr) at ({-1*\mxoff}, {-1*\myoff}) {Dwarf shrubs};
  \node[TolRbwF, rll node] (lsgras) at ({2*\mxoff}, {-2.5*\myoff}) {LS grassland};
  \node[TolRbwF, rll node] (shoher) at ({1.*\mxoff}, {-2.5*\myoff}) {Short herbs};
  \node[TolRbwJ, rll node] (chinop) at ({3*\mxoff}, {-3*\myoff}) {Chinopholous vegetation};
    \path[pil]
  (domgra) edge[drP, bend right=25] (hsforb.west)
  (dwashr) edge[drP, bend left=10] (hsforb)
  (msgras) edge[drN, bend right=25] (hsforb.east)  
  (msgras) edge[drN, bend left=25] (lsgras)
  (msgras) edge[drN, bend left=25] (chinop)
  (lsgras) edge[drN, in=65,out=115,looseness=1] (shoher)
  (msgras) edge[drN, in=175,out=190,looseness=5] (msgras)
  (shoher) edge[drP, in=175,out=190,looseness=5] (shoher)
  (chinop) edge[drP, in=175,out=190,looseness=5] (chinop);
  % \node[rel node, yshift=2.5pt] (Emsgras) at (msgras.south) {Fest Viol, Trif spp};  
  % \node[rel node, yshift=2.5pt] (Ehsforb) at (hsforb.south) {Minuartia verna};
  % \node[rel node, yshift=0pt] (Edomgra) at (domgra.south) {Kobresia spp , Carex Spp};
  % \node[rel node, yshift=2.5pt] (Edwashr) at (dwashr.south) {Salix herbacea};
  % \node[rel node, yshift=2.5pt] (Elsgras) at (lsgras.south) {Alch glau, Anth nipp};
  % \node[rel node, yshift=2.5pt] (Eshoher) at (shoher.south) {Plantago alpina};
  % \node[rel node, yshift=0pt] (Echinop) at (chinop.south) {Carex foetida};
  %%%%%%%%%%%%% 
  \node[TolRbwA, rel node, yshift=2.5pt] (Emsgras) at (msgras.south) {Fest Viol, Trif spp};  
  \node[TolRbwA, rel node, yshift=2.5pt] (Ehsforb) at (hsforb.south) {Minuartia verna};
  \node[TolRbwA, rel node, yshift=0pt] (Edomgra) at (domgra.south) {Kobresia spp, Carex Spp};
  \node[TolRbwD, rel node, yshift=2.5pt] (Edwashr) at (dwashr.south) {Salix herbacea};
  \node[TolRbwF, rel node, yshift=2.5pt] (Elsgras) at (lsgras.south) {Alch glau, Anth nipp};
  \node[TolRbwF, rel node, yshift=2.5pt] (Eshoher) at (shoher.south) {Plantago alpina};
  \node[TolRbwJ, rel node, yshift=0pt] (Echinop) at (chinop.south) {Carex foetida};
  % \node[rel node, yshift=2.5pt] (Emsgras) at (msgras.south) {\textcolor{TolRbwA}{Fest Viol, Trif spp}};  
  % \node[rel node, yshift=2.5pt] (Ehsforb) at (hsforb.south) {\textcolor{TolRbwA}{Minuartia verna}};
  % \node[rel node, yshift=0pt] (Edomgra) at (domgra.south) {\textcolor{TolRbwA}{Kobresia spp, Carex Spp}};
  % \node[rel node, yshift=2.5pt] (Edwashr) at (dwashr.south) {\textcolor{TolRbwD}{Salix herbacea}};
  % \node[rel node, yshift=2.5pt] (Elsgras) at (lsgras.south) {\textcolor{TolRbwF}{Alch glau, Anth nipp}};
  % \node[rel node, yshift=2.5pt] (Eshoher) at (shoher.south) {\textcolor{TolRbwF}{Plantago alpina}};
  % \node[rel node, yshift=0pt] (Echinop) at (chinop.south) {\textcolor{TolRbwJ}{Carex foetida}};

\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "tikz_figures"
%%% End:


==> results.tex <==
\newpage

\section{Results}

\subsection{Experiment 1}


\subsection{Experiment 2}
 



\subsection{Plant associations along an Alpine mesotopographic gradient}
\subsection{Plant associations along an Alpine mesotopographic gradient}
%\subsubsection{Plant habitat suitability}
%% No difference in AUC between HSM only and full HSM
%\subsubsection{Plant associations along the mesotopographic gradient}
The application of our approach to the Alpine dataset identified four densely connected modules of different sizes, within which species occupied distinct structural roles in the plant association network. Modules were structured along the snow melting date gradient (Fig.~\ref{assocplant:a}). 

Species from early-melting sites were classified into the same module. We found a prominence of positive associations, specifically an unselective mostly asymmetric attraction of forbs and grasses to tall dominant graminoids (\textit{Carex, Kobresia}).  Instead, forbs and grasses formed two distinct groups  linked by negative associations. Besides, some of them acted as hubs connecting the high elevation sites to the adjacent sites where they also occurred. The second module encompassed two groups of grasses: (i) Tall herbs occurring in favorable conditions, mostly structured by negative associations (ammensalism and competition); (ii) Short herb meadows, exposed to zoogenic disturbances. They presented higher abundances when co-occurring with tall herbs. The third module consisted of chinopholous (cold-resistant) vegetation appearing on late-melting sites. The last module included north-facing isolated communities dominated by \textit{Salix herbacea} positively associated with high-altitude communities, but disconnected from the other modules (Fig.~\ref{assocplant}).

Interestingly, we found more positive associations in communities from stressful conditions like early melting sites where species are exposed to wind and erosion due to snow melting \cite{choler2005consistent}. The positive associations could be explained by the facilitative effect of graminoids through multiple hypothetical mechanisms. Graminoids have the ability to maintain the soil stability \cite{callaway2007positive,heilbronn1984plant}, they can also prevent dessication and frost heaving on stones in favor of seedling survival \cite{choler2001facilitation}. They also sustain a suitable microclimate for small forbs and grasses, while offering protection from the wind \cite{wardle1998can}. On the other hand, negative associations were found in the species rich sites, which are likely the outcome of 
competition for resources: water and Nitrogen \cite{choler2001facilitation}.

%% On the structure of the network and its drivers %%
As reported in the literature, the abiotic conditions strongly structured the predicted response \cite{choler2005consistent} of the plant species and the dominant interaction types \cite{callaway2002positive}. Specifically, network modules were distributed along the gradient following their composition's response to the average snow duration. Negative associations inflicted by competitive tall grasses on mid slope communities connected early-melting communities to the chinopholous vegetation from late-melting sites in the resulting association network (Fig.~\ref{assocplant:b}). Response and effect groups were included in one or at most two close (in terms of position in the gradient) modules (Fig.~\ref{assocplant:a}). Non neutral associations had consistent types (either negative or positive) within effect groups regardless of the responding species, suggesting that species roles (effects) in their community might be predictable from their own characteristics and the surrounding abiotic conditions. At last, learnt associations were symmetric within groups but asymmetric (mostly semi-attraction or semi-repulsion) between them.   

%%TC:ignore
\begin{figure}[H]
	\begin{subfigure}{\textwidth}
		\centering
		\includegraphics[scale=0.15]{images/assoc_clustermap.pdf}
		\caption{Inferred plant association matrix. Species in the association matrix are grouped based on a hierarchical bi-clustering performed row-wise (yielding response groups) and column-wise (yielding effect groups).} \label{assocplant:a}
	\end{subfigure}
	\newline
	\centering
	\begin{subfigure}{\textwidth}
		\includegraphics[scale=0.4]{images/network.PNG}
		\caption{Network of plant associations. Blue (resp.\ red) edges indicate negative (resp.\ positive) edge weights. Node colors on the graph represent communities identified by the modularity maximization algorithm \cite{newman2006modularity} whilst node sizes are scaled according to the plant height. Nodes (except \textit{Salix herbacea}, which represents the vegetation on the northern face of the gradient) are placed from left to right following an ascending order of their response to Snow duration (regression coefficient from the Generalized Linear Model used as a Habitat Suitability Model).  } \label{assocplant:b}
	\end{subfigure}
	\newline
	\centering
	\caption{Plant associations on an Alpine mesotopographic gradient. We highlight the communities (node colors) in figure (b) using colored labels on the matrix (a). } \label{assocplant}
\end{figure}
%\
%%TC:endignore







==> scatter_AlpsPlantScores.tex <==
\renewcommand{\datafile}{xps/data_AlpsPlantScores.csv}

\tikzstyle{every pin}=[font=\footnotesize, inner sep = 1pt]
\tikzstyle{every pin edge}=[thin, lightgray]

\begin{tikzpicture}[node distance=.2em]%[trim axis left, trim axis right]
\draw[opacity=0] (-.8,-.1) rectangle ++(\textwidth, 6.2);
\pgfmathsetmacro{\factX}{11}\pgfmathsetmacro{\offX}{0}%
\pgfmathsetmacro{\vXmin}{0.38}\pgfmathsetmacro{\vXmax}{.93}%
\pgfmathsetmacro{\factY}{6}\pgfmathsetmacro{\offY}{0}%
\pgfmathsetmacro{\vYmin}{0.65}\pgfmathsetmacro{\vYmax}{1.06}%

\node[anchor=south, rotate=90, font=\footnotesize] at ({-.05*\factX},{.5*\factY}) {ROC AUC};

\pgfmathsetmacro{\marky}{\factY*(1-\vYmin)/(\vYmax-\vYmin)}%
\draw[thin, dotted, darkgrey] (0,\marky) -- ++({\factX+.2},0);

\pgfmathsetmacro{\marky}{\factY*(0.91-\vYmin)/(\vYmax-\vYmin)}%
%\path (0,0) edge ({\factX+.2},0);
\path (0,0) edge (0,{\marky});
\foreach \l in {0.7, 0.8, 0.9}{
  \pgfmathsetmacro{\marky}{\factY*(\l-\vYmin)/(\vYmax-\vYmin)}%
  \draw (-.05,\marky) -- ++(.1,0);
  \draw[thin, dotted, darkgrey] (0,\marky) -- ++({\factX+.2},0);
  \node[anchor=east, font=\footnotesize] at (-.06, \marky) {$\l$};
}

\csvreader[head to column names]{\datafile}{}{%
  %\pgfmathsetmacro{\markx}{\factX*(sqrt(\prevalence+\avgcountnz)-\vXmin)/(\vXmax-\vXmin)}%
  \pgfmathsetmacro{\markx}{\factX*(sqrt(sqrt(\prevalence))-\vXmin)/(\vXmax-\vXmin)}%
  \pgfmathsetmacro{\marky}{\factY*(\score-\vYmin)/(\vYmax-\vYmin)}%
  %\node[pnt node, TolRbw\gcl, pin={[pin distance = \pndst em] \pngl:{\genus}}] at (\markx,\marky) {};
  \node[pnt node, black, pin={[pin distance = \pndst em] \pngl:{\slbl}}] at (\markx,\marky) {};
  %\node[pnt node, TolRbw\gcl, font=\tiny, pin={[pin distance = .8em] {\pngl+\thecsvrow/15}:{\thecsvrow}}] at (\markx,\marky) {};
}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "tikz_figures"
%%% End:

